Primal-dual gap estimators for a posteriori error analysis of nonsmooth minimization problems

The primal-dual gap is a natural upper bound for the energy error and, for uniformly convex minimization problems, also for the error in the energy norm. This feature can be used to construct reliable primal-dual gap error estimators for which the constant in the reliability estimate equals one for the energy error and equals the uniform convexity constant for the error in the energy norm. In particular, it defines a reliable upper bound for any functions that are feasible for the primal and the associated dual problem. The abstract a posteriori error estimate based on the primal-dual gap is provided in this article, and the abstract theory is applied to the nonlinear Laplace problem and the Rudin-Osher-Fatemi image denoising problem. The discretization of the primal and dual problems with conforming, low-order finite element spaces is addressed. The primal-dual gap error estimator is used to define an adaptive finite element scheme and numerical experiments are presented, which illustrate the accurate, local mesh refinement in a neighborhood of the singularities, the reliability of the primal-dual gap error estimator and the moderate overestimation of the error.

==> includes/header_include.tex <==
\usepackage{ifthen}
\ifthenelse{\equal{\users}{world}}{}{
  \usepackage{fancyhdr}
  \pagestyle{fancy}
  \topmargin=-.0cm
  \headheight=28pt
  \definecolor{darkgrey}{RGB}{144,144,144}
  \rhead{\color{darkgrey} \header}
  \chead{}
 \lhead{\color{darkgrey}Version \version, file: \jobname.tex \\
   compiled: % \today
   \number\day.\number\month.\number\year\ at
   \the\hour:\ifnum\minute<10 0\fi\the\minute\ h }
}
\newcount\hour \newcount\minute
\hour=\time 
\divide \hour by 60
\minute=\time
\loop \ifnum \minute > 59 \advance \minute by -60 \repeat


==> misc.tex <==
\section{Relation between Primal-Dual Algorithm and ADMM}

We consider the minimization of the functional
\begin{align*}
E(u_h) = F(\nabla u_h) + G(u_h) = \int_\O |\nabla u_h| \dv{x} + \frac{\a}{2} \|u_h-g\|^2
\intertext{and the corresponding saddle-functional}
S(u_h,p_h) = \int_\O \nabla u_h \cdot p_h \dv{x} + \frac{\a}{2}\|u_h-g\|^2 - I_{K_1(0)}(p_h).
\end{align*}
To approximate a saddle-point we consider discrete (sub-)gradient flows in descent direction
with respect to the variable ~$u_h$ and in ascent direction with respect to ~$p_h$.

\begin{algorithm}[Primal-dual algorithm]
Set $u_h^{-1}=u_h^0=0$, $p_h^0=0$ and $k=0$.\\
(1) Set $\til{u}_h^{k+1} = 2u_h^k - u_h^{k-1}$.\\
(2) Compute $p_h^{k+1} \in \cL^0(\cT_h)$ such that
\[
p_h^{k+1} = \operatorname{argmin}_{p_h} -(\nabla \til{u}_h^{k+1},p_h) +
F^*(p_h) + \frac{1}{2 \tau} \|p_h-p_h^k\|^2.
\]
(3) Compute $u_h^{k+1} \in \cS^1(\cT_h)$ such that
\[
u_h^{k+1} = \operatorname{argmin}_{u_h} (\nabla u_h,p_h^{k+1}) +
G(u_h) + \frac{1}{2 \tau} \|u_h-u_h^k\|_h^2.
\]
(4) Stop if stopping criterion is satisfied. Otherwise set $k=k+1$ and continue with ~(1).
\end{algorithm}

Here, the norm $\|\cdot\|_h$ is either $\|v_h\|_h=\|v_h\|$ or $\|v_h\|_h^2=\|v_h\|^2 + h\|\nabla v_h\|^2$.\\
\\
The approach of ADMM (or ALG 2 in Glowinski/Fortin) is slightly different since it does not use
Fenchel conjugates. We introduce the auxiliary variable $q_h=\nabla u_h$ and enforce this
relation by a Lagrange multiplier $\l_h \in \cL^0(\cT_h)$ and a penalization term which
yields the following saddle-functional:
\[
L(u_h,q_h;\l_h) = \int_\O |q_h| \dv{x} + \frac{\a}{2}\|u_h-g\|^2 +
(\l_h,q_h-\nabla u_h)_w + \frac{\s}{2}\|q_h-\nabla u_h\|_w^2.
\]
Here, the norm ~$\|\cdot\|_w$ is the weighted $L^2$-norm $\|\mu_h\|_w=h^{\g/2} \|\mu_h\|$
with either $\g=0$ or $\g=d$.
The ADMM then performs an alternate minimization with respect to the variables ~$u_h$ and
~$q_h$ and an ascent step with respect to $\l_h$:

\begin{algorithm}[ADMM]
Set $\l_h=0$ and $u_h^0=0$ and $k=0$.\\
(1') Compute $q_h^{k+1} \in \cL^0(\cT_h)$ such that
\[
q_h^{k+1} = \operatorname{argmin}_{q_h} F(q_h) + (\l_h^k,q_h)_w +
\frac{\s}{2} \|q_h-\nabla u_h^k\|_w^2.
\]
(2') Compute $u_h^{k+1} \in \cS^1(\cT_h)$ such that
\[
u_h^{k+1} = \operatorname{argmin}_{u_h} G(u_h) - (\l_h^k,\nabla u_h)_w +
\frac{\s}{2} \|q_h^{k+1}-\nabla u_h\|_w^2.
\]
(3') Set
\[
\l_h^{k+1} = \l_h^k + \s(q_h^{k+1}-\nabla u_h^{k+1})
\]
(4) Stop if stopping criterion is satisfied. Otherwise, set $k=k+1$ and continue with ~(1').
\end{algorithm}

The minimality property of ~$q_h^{k+1}$ in ~\textit{(1')} is equivalent to
\begin{align*}
&\; 0 \in \partial F(q_h^{k+1}) + h^\g( \l_h^k + \s (q_h^{k+1}-\nabla u_h^k)) \\
\Leftrightarrow \quad &\; \underbrace{h^\g(-\l_h^k - \s (q_h^{k+1}-\nabla u_h^k))}_{=h^\g(-\l_h^{k+1}-\s (\nabla u_h^{k+1}-\nabla u_h^k))} \in \partial F(q_h^{k+1}) \\
\Leftrightarrow \quad &\; \underbrace{q_h^{k+1}}_{=\frac{\l_h^{k+1}-\l_h^k}{\s}+\nabla u_h^{k+1}} \in \partial F^*(h^\g(-\l_h^{k+1} - \s (\nabla u_h^{k+1}-\nabla u_h^k))) \\
\Leftrightarrow \quad &\; -\l_h^k + \s \nabla u_h^{k+1} \in -\l_h^{k+1} + \s \partial F^*(h^\g(-\l_h^k - \s (\nabla u_h^{k+1}-\nabla u_h^k))) \\
\Leftrightarrow \quad &\; h^\g(-\l_h^k + \s \nabla u_h^{k+1} - \s(\nabla u_h^{k+1}-\nabla u_h^k)) \in \underbrace{h^\g(-\l_h^{k+1} -\s(\nabla u_h^{k+1}-\nabla u_h^k))}_{=:p_h^{k+1}}\\
& \qquad \qquad \qquad +h^\g\s \partial F^*(\underbrace{h^\g(-\l_h^k - \s (\nabla u_h^{k+1}-\nabla u_h^k))}_{=p_h^{k+1}}) \\
\Leftrightarrow \quad &\; p_h^{k+1} = (I+\s h^\g \partial F^*)^{-1}\underbrace{(h^\g(-\l_h^k+\s\nabla u_h^k))}_{=h^\g (-\l_h^k-\s(\nabla u_h^k - \nabla u_h^{k-1})) +h^\g \s(2\nabla u_h^k - \nabla u_h^{k-1})} \\
& \qquad \quad = (I+\s h^\g \partial F^*)^{-1}(p_h^k+\s h^\g \nabla \til{u}_h^{k+1})\underset{\text{if } \s h^\g=\tau}{=}\textit{(2)}.
\end{align*}
In particular, with the definition of $p_h^k$, we have
\begin{equation}
\begin{split}
q_h^{k+1} &= \frac{\l_h^{k+1}-\l_h^k}{\s} + \nabla u_h^{k+1} \\
&= \frac{-p_h^{k+1}-\s(\nabla u_h^{k+1}-\nabla u_h^k)+p_h^k + \s (\nabla u_h^k-\nabla u_h^{k-1})}{\s} + \nabla u_h^{k+1} \\
&= \frac{p_h^k - p_h^{k+1}}{\s} + 2 \nabla u_h^k - \nabla u_h^{k-1}.
\end{split}
\end{equation}
Next, we consider only $\g=0$. We modify the minimization in ~\textit{(2')} as follows:
\begin{align*}
u_h^{k+1} &= \operatorname{argmin}_{u_h} G(u_h) - (\l_h^k,\nabla u_h) +
\frac{\s}{2} \|q_h^{k+1}-\nabla u_h\|^2 \\
&\; + \frac{1}{2\tau}\|u_h-u_h^k\|_h^2 - \frac{\s}{2}\|\nabla(u_h-u_h^k)\|^2 \\
&=  \operatorname{argmin}_{u_h} G(u_h) - (\l_h^k,\nabla u_h) + \frac{\s}{2}\|\nabla u_h\|^2 - \s(q_h^{k+1},\nabla u_h)\\
&\; + \frac{1}{2\tau}\|u_h-u_h^k\|^2 - \frac{\s}{2}\|\nabla u_h\|^2 + \s(\nabla u_h,\nabla u_h^k)\\
&= \operatorname{argmin}_{u_h} G(u_h) - (\diver(p_h^k+\s(\nabla u_h^k-\nabla u_h^{k-1}),u_h) \\
& \; + (\s \diver q_h^{k+1},u_h) + \frac{1}{2\tau}\|u_h-u_h^k\|^2 - (u_h,\s \diver\nabla u_h^k) \\
&=  \operatorname{argmin}_{u_h} G(u_h) + \frac{1}{2\tau}\|u_h-u_h^k\|^2 \\
&\; - (\diver(\underbrace{p_h^k+2\s\nabla u_h^k-\s\nabla u_h^{k-1}-\s q_h^{k+1}}_{=p_h^{k+1}}),u_h) \\
&=  \operatorname{argmin}_{u_h} G(u_h) + (p_h^{k+1},\nabla u_h)  + \frac{1}{2\tau}\|u_h-u_h^k\|^2
\end{align*}
which is ~\textit{(3)}. The modified minimization problem is well-defined if the
additional term is coercive which is the case for $\tau \s < h$. Choosing
$\tau=\s$ we obtain $\tau=\mathcal{O}(h^{1/2})$.

\medskip
\textit{Acknowledgements.} The authors acknowledge financial support for the project "Finite Element approximation of functions of bounded variation and application to model of damage, fracture and plasticity" (BA 2268/2-1) by the DFG via the priority program "Reliable Simulation Techniques in Solid Mechanics, Development of Non-standard Discretization Methods, Mechanical and Mathematical Analysis" (SPP 1748).

